Complete asymptotic type-token relationship for growing complex systems with inverse power-law count rankings

The growth dynamics of complex systems often exhibit statistical regularities involving power-law relationships. For real finite complex systems formed by countable tokens (animals, words) as instances of distinct types (species, dictionary entries), an inverse power-law scaling $S \sim r^{-\alpha}$ between type count $S$ and type rank $r$, widely known as Zipf's law, is widely observed to varying degrees of fidelity. A secondary, summary relationship is Heaps' law, which states that the number of types scales sublinearly with the total number of observed tokens present in a growing system. Here, we propose an idealized model of a growing system that (1) deterministically produces arbitrary inverse power-law count rankings for types, and (2) allows us to determine the exact asymptotics of the type-token relationship. Our argument improves upon and remedies earlier work. We obtain a unified asymptotic expression for all values of $\alpha$, which corrects the special cases of $\alpha = 1$ and $\alpha \gg 1$. Our approach relies solely on the form of count rankings, avoids unnecessary approximations, and does not involve any stochastic mechanisms or sampling processes. We thereby demonstrate that a general type-token relationship arises solely as a consequence of Zipf's law.

==> makepackage <==
#!/bin/sh
echo "creating $1-arxiv.tgz..." 1>&2;
cd package;

mkdir -p anc

\cp ~/work/stories/2020-08gutenberg-jane-austen/figures/figallotaxonometer9000-jane-austen-1grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-1-probability-divergence-pride-and-prejudice-1-grams.pdf
\cp ~/work/stories/2020-08gutenberg-jane-austen/figures/figallotaxonometer9000-jane-austen-2grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-2-probability-divergence-pride-and-prejudice-2-grams.pdf
\cp ~/work/stories/2020-08gutenberg-jane-austen/figures/figallotaxonometer9000-jane-austen-3grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-pride-and-prejudice-3-grams.pdf

\cp ~/work/stories/2020-01story-wrangler-rtd/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-1grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-twitter-1-grams.pdf
\cp ~/work/stories/2020-01story-wrangler-rtd/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-2grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-twitter-2-grams.pdf
\cp ~/work/stories/2020-01story-wrangler-rtd/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-3grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-twitter-3-grams.pdf

\cp ~/work/ecology/2019-11barro-colorado-trees-35-years/figures/figallotaxonometer9000-1985-2015-barro-colorado003-ptd-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-7-probability-turbulence-divergence-barro-colorado-island.pdf


\cp anc/allotaxonometer-flipbook-1-probability-divergence-pride-and-prejudice-1-grams.pdf \
    flipbooks/S1-flipbook-probability-divergence.pdf
    
\cp anc/allotaxonometer-flipbook-2-probability-divergence-pride-and-prejudice-2-grams.pdf \
    flipbooks/S2-flipbook-probability-divergence.pdf
    
\cp anc/allotaxonometer-flipbook-3-probability-divergence-pride-and-prejudice-3-grams.pdf \
    flipbooks/S3-flipbook-probability-divergence.pdf

\cp anc/allotaxonometer-flipbook-4-probability-divergence-twitter-1-grams.pdf \
    flipbooks/S4-flipbook-probability-divergence.pdf
    
\cp anc/allotaxonometer-flipbook-5-probability-divergence-twitter-2-grams.pdf \
    flipbooks/S5-flipbook-probability-divergence.pdf
    
\cp anc/allotaxonometer-flipbook-6-probability-divergence-twitter-3-grams.pdf \
    flipbooks/S6-flipbook-probability-divergence.pdf
    

\cp anc/allotaxonometer-flipbook-7-probability-turbulence-divergence-barro-colorado-island.pdf \
    flipbooks/S7-flipbook-probability-divergence.pdf
    



tar cvfzph ../$1-arxiv.tgz fig[0-9]*.pdf *revtex4-combined.tex anc/* 1>&2;



==> makepackage-arxiv <==
#!/bin/sh
echo "creating $1-arxiv.tgz..." 1>&2;

cd package;

mkdir -p anc

# clean anything if there
\rm anc/*


# jane austen
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-1grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-1-probability-divergence-pride-and-prejudice-1-grams.pdf
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-2grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-2-probability-divergence-pride-and-prejudice-2-grams.pdf
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-3grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-pride-and-prejudice-3-grams.pdf

# twitter
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-1grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-4-probability-divergence-twitter-1-grams.pdf
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-2grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-5-probability-divergence-twitter-2-grams.pdf
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-3grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-6-probability-divergence-twitter-3-grams.pdf

# barro colorado island
\cp ../figures/2019-11barro-colorado-trees-35-years/flipbooks/figallotaxonometer9000-1985-2015-barro-colorado003-ptd-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-7-probability-turbulence-divergence-barro-colorado-island.pdf

## tar cvfzph ../$1-arxiv.tgz fig[0-9][0-9]*.pdf *revtex4-combined.tex anc/ 1>&2;
tar cvfzph ../$1-arxiv.tgz fig[0-9][0-9]*.pdf *revtex4-combined.tex 1>&2;

cd ..



==> makepackage-no-bibtex <==
#!/bin/sh
echo "creating $1-arxiv.tgz..." 1>&2;

cd package;

mkdir -p anc

# clean anything if there
\rm anc/*


# jane austen
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-1grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-1-probability-divergence-pride-and-prejudice-1-grams.pdf
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-2grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-2-probability-divergence-pride-and-prejudice-2-grams.pdf
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-3grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-pride-and-prejudice-3-grams.pdf

# twitter
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-1grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-4-probability-divergence-twitter-1-grams.pdf
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-2grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-5-probability-divergence-twitter-2-grams.pdf
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-3grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-6-probability-divergence-twitter-3-grams.pdf

# barro colorado island
\cp ../figures/2019-11barro-colorado-trees-35-years/flipbooks/figallotaxonometer9000-1985-2015-barro-colorado003-ptd-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-7-probability-turbulence-divergence-barro-colorado-island.pdf

## tar cvfzph ../$1-arxiv.tgz fig[0-9][0-9]*.pdf *revtex4-combined.tex anc/ 1>&2;
tar cvfzph ../$1-arxiv.tgz fig[0-9][0-9]*.pdf *revtex4-combined.tex 1>&2;

cd ..



==> package-arxiv <==
#!/bin/sh
echo "creating probability-divergence-manuscript-arxiv.tgz..." 1>&2;

tar cvfzph \
    probability-divergence-manuscript-arxiv.tgz \
    probability-divergence-manuscript.tex \
    probability-divergence-manuscript.*.tex \
    probability-divergence-manuscript.bbl \
    probability-divergence.*.tex \
    probability-divergence.bib \
    figures/localized/*





==> simple-derivation-of-the-finite-type-token-law-revtex4.settings.tex <==
\newcommand{\filenamebase}{simple-derivation-of-the-finite-type-token-law}


==> simple-derivation-of-the-finite-type-token-law.biblio.tex <==
\bibliography{\filenamebase}


==> simple-derivation-of-the-finite-type-token-law.body_old.tex <==
%% !!! no latex settings inside .body.tex or any content files

% \section{Introduction}
% \label{sec:simple-type-token.introduction}

\begin{textblock}
\item 
  \textit{Introduction}---Universal statistical regularities play a central role in the study of complex systems.
\item 
  Prominent examples are power-law relationships, 
  such as Zipf’s law for word frequencies~\cite{zipf1949a,newman2005b},
\item 
  observed across human~\cite{altmann2016} and animal~\cite{arnon2025} communication. 
\item 
  For language, Zipf’s law states that the count of a word
  in a text decreases with its rank $r$ as
  $S_{\rank,\rankdistexponent} \sim r^{-\rankdistexponent}$, 
  originally with $\rankdistexponent \simeq 1$.
\item 
  While arguments about 
  the empirical validity and mechanistic origins 
  of Zipf's law have remained contentious for the 
  better part of a century~\cite{yule1925,mandelbrot1953a,simon1955a,maillart2008a,ferrericancho2010a,williams2015b},
\item 
  count-rankings adhering approximately to an inverse power-law have been observed across systems 
  of all kinds including
  ecological systems~\cite{yule1925, camacho2001}, 
  complex networks~\cite{Redner1998, barabasi1999},  
  and socioeconomic systems~\cite{serrano2003,pinto2012, gabaix2016,gaillard2023}. 
\end{textblock}

\begin{textblock}
\item 
  Another well-known scaling regularity is Heaps’
  law~\cite{herdan1960,heaps1978,Chacoma2020},  
\item
  which describes how the vocabulary count $N$ of a text grows with its total length $t$ as $N_{t, \beta} \sim t^{\beta}$,  with $0 < \beta < 1$. 
\item
  Like Zipf's law,
  type-token scaling has been found to generalize beyond language,
  and has been reported to hold in, for example,
\item
  chemoinformatics~\cite{benz2008},
  computer code~\cite{zhang2009},
  and urban systems~\cite{simini2019}.
\item 
 The type-token relationship is a summary one,
 as it carries far less information than count ranking
 which records not just type ranks but the names
 of the types themselves. 
 %(if often omitted in figures).
\end{textblock}

\begin{textblock}
\item 
The fact that Zipf’s and Heaps’ laws are empirically observed to hold simultaneously has motivated interest in whether or not a fundamental relationship between them exists in finite, real systems. 
\item
Previous works have developed a range of frameworks to relate both scaling laws, for example, by
\item
empirical observation~\cite{baeza-yates2000}, 
\item
proposing specific language models~\cite{zanette2005,serrano2009}, 
\item
growth dynamics~\cite{laurent2016},
\item
sampling mechanisms~\cite{vanleijenhorst2005, eliazar2011}, 
\item
or assuming in advance their simultaneous validity~\cite{bernhardsson2009}.
\item
L\"{u} \textit{et al.}~\cite{lu2010a}, whose work we improve upon,
found
that the scaling relation between the two exponents in the infinite system count
limit is given by
\item
\begin{equation}
    \beta = 
    \begin{cases}
        1
        & 
        \textnormal{for} 
        \ 
        \alpha \le 1,
        \\
             1/\alpha
        & 
        \textnormal{for} 
        \ 
        \alpha > 1.
    \end{cases}
    \label{eq:simple-type-token.lu-exponents}
\end{equation}
\end{textblock}

\begin{textblock}
\item
In this work, we derive a complete asymptotic type–token relationship for idealized growing finite systems, valid for any value of the scaling exponent 
$0 \leq \alpha < \infty$.
\item
Our formulation corrects earlier approximations
and returns the scaling form of Heaps' law in specific limits.
\item
Our approach is independent of the underlying mechanisms of the system, provides an excellent fit to our growing system model, and offers further insight into the growth dynamics of real systems.
\end{textblock}


% \section*{Model of \\an idealized growing system}
% \label{sec:simple-type-token.model}

\begin{textblock}
\item
  \textit{Model of an idealized growing system}---We consider an idealized growing system comprising
  countable tokens as instances of types. 
\item
  We set aside physical mechanisms
  and consider a system emerging
  in time as follows.
\item
  The system grows in discrete time  
  so that there are $\rgrtime$ total
  tokens at time $\rgrtime = 1, 2, 3,   \ldots$,
  and such that the count of
  the $\rank$th type is
\item
  \begin{equation}
    \typesize_{\rank,\rgrtime,\rankdistexponent}
    =
    \left\lfloor
    \frac{1}{2}
    +
    \growthfactor
    \rank^{-\rankdistexponent}
    \right\rfloor,
    \label{eq:simple-type-token.Srt-base-equation-set-up}
  \end{equation}
\item
  where 
  $\rankdistexponent > 0$,
  $\lfloor \cdot \rfloor$
  is the floor operator, converted to a round-to-the-nearest-integer
  operator by the addition of 1/2, 
  and $\growthfactor$ is a growth factor
  which we define below.
\item
  We indicate count by $\typesize$ which stands
  for the more general conception of size.
\item
  For $\rankdistexponent = 0$,
  $
  \typesize_{\rank,\rgrtime,0}
  =
  1
  $
  for 
  $1 \le \rank \le t$
  and 
  0
  otherwise.
\item
  By construction, types remain ordered in count ranking
  according to their arrival time.
\item
  When the $\rank$th type's
  count
  $\typesize_{\rank,\rgrtime,\rankdistexponent}$
  first
  rounds up to 1 (i.e., reaches $1/2$),
  we may consider the type 
  as being created or uncovered.
\item
  At any time $t$, there will be a finite number
  $\Ndistincttypesfn{\rgrtime}{\rankdistexponent}$
  of
  types with one or more tokens in the system, $\Ndistincttypesfn{\rgrtime}{\rankdistexponent}$
  being also the rank of
  the most recently arrived type.
\item
  Because the system is a realized entity,
  we call 
  $\typesize_{\rank,\rgrtime,\rankdistexponent}$
  a count-ranking rather than a count-rank distribution,
  which mis-implies, for our model, a sampling process.
\end{textblock}

\begin{textblock}
\item 
  The growth factor
  $\growthfactor \ge 0$
  ``grows'' the system in a step-wise fashion so that
\item 
  \begin{equation}
    \rgrtime
    =
    \sum_{\rank=1}^{\infty}
    \left\lfloor
     \frac{1}{2}
     +
    \growthfactor
    \rank^{-\rankdistexponent}
    \right\rfloor.
    \label{eq:simple-type-token.Srt-base-equation-set-up-prefactor}
  \end{equation}
  
\item
 Equation~\eqref{eq:simple-type-token.Srt-base-equation-set-up-prefactor} means that, for a given value of $t$, there will be an increasingly small range of 
 values of $\growthfactor$ for which $t$ tokens are present in the system.
\item 
 Also, not all individual token counts $t$ are achievable, 
 because two types can reach a half integer
 simultaneously.
\end{textblock}

\begin{textblock}
\item
  Now, while our idealized system can be easily grown computationally,
  the floor operator prevents ready analysis.
\item
  We approximate the count-ranking of our model as
\item
  \begin{equation}
    \typesize_{\rank,\rgrtime,\rankdistexponent}
    =
    \left\{
    \begin{array}{ll}
      \typesize_{1,\rgrtime,\rankdistexponent}
      \rank^{-\rankdistexponent}
      &
      \textnormal{for}
      \quad
      1
      \le
      \rank
      \le
      \Ndistincttypes,
      \\
      0
      &
      \textnormal{for}
      \quad
      \rank
      >
      \Ndistincttypes.
    \end{array}
    \right.
    \label{eq:simple-type-token.Srt-approx}
  \end{equation}
  
\item
  Counts are now fractional,
  and we determine 
  $\typesize_{1,\rgrtime,\rankdistexponent}$ 
  below.
\item 
  We note that in some limits, the approximation may not allow
  us to capture the idealized system,
  particularly as $\alpha \rightarrow 0$, because the continuous form smooths over the discrete, step-wise growth that dominates when the count hierarchy flattens, causing the approximate scaling to fail to represent the actual ranked increments.
\item
  Nevertheless, we will be able to satisfactorily
  connect count-rank scaling
  to type-token scaling.
\end{textblock}

\begin{textblock}
\item
  To maintain the connection to our idealized base model, we enforce two conditions.
\item
  First, when a type first appears it has a count of 1.
\item  
  Setting rank $\rank$ to $\Ndistincttypes$
  in Eq.~\eqref{eq:simple-type-token.Srt-approx},
  we have
\item
  \begin{equation}
    \typesize_{\Ndistincttypes,t,\rankdistexponent}
    =
    1
    =
    \typesize_{1,\rgrtime,\rankdistexponent}
    \Ndistincttypes^{-\rankdistexponent},
    \label{eq:simple-type-token.S1-scaling-set-up}
  \end{equation}
\item
  which means
\item 
  \begin{equation}
    \typesize_{1,\rgrtime,\rankdistexponent}
    \sim
    \Ndistincttypes^{\rankdistexponent}.
    \label{eq:simple-type-token.S1-scaling}
  \end{equation}
\item
  Second, we must have the sum of fractional counts equal to time $\rgrtime$, so
\item 
  \begin{equation}
    \rgrtime
    =
    \sum_{\rank=1}^{N}
    \typesize_{\rank,\rgrtime,\rankdistexponent}
    \sim 
    \Ndistincttypes^\rankdistexponent, 
    \genharmonicsum{\Ndistincttypes}{\rankdistexponent}
    \label{eq:simple-type-token.type-token-relationship}
  \end{equation}
\item 
where
\begin{equation}
    \genharmonicsum{n}{a} 
    =
    \sum_{k=1}^{n} 
    k^{-a}
\end{equation}
\item
is the $n$th generalized harmonic number
of order $a$.
\item
  Eq.~\eqref{eq:simple-type-token.type-token-relationship} implicitly gives us what we call
  the type-token relationship, i.e.,
  how the number of distinct types $\Ndistincttypes$ grows with the 
  overall number tokens, $\rgrtime$. 
\item 
    We may approximate the harmonic sum in Eq.~\eqref{eq:simple-type-token.type-token-relationship} by its integral form,
    \begin{equation}
    \genharmonicsum{\Ndistincttypes}{\rankdistexponent} 
    \sim 
    \int_{z=1}^{\Ndistincttypes}
    z^{-\rankdistexponent}
    \dee{z},
    \label{eq:simple-type-token.genharmonicsum-approx}
    \end{equation}
    so we would arrive to
    \begin{equation}
        t \sim \frac{
      \Ndistincttypes^{\rankdistexponent}
    }{
      1 - \rankdistexponent
    }
    \left[
      \Ndistincttypes^{1-\rankdistexponent}
      -
      1
      \right].
      \label{eq:simple-type-token.integral_approximation_Lu}
    \end{equation}
    
\item    Equation~\eqref{eq:simple-type-token.integral_approximation_Lu} coincides with the result obtained by L\"{u}~\textit{et}~\textit{al.}\ in Ref.~\cite{lu2010a}, where the authors derive the connection between the number of distinct types and the total number of tokens by transforming their count-ranking into a size-frequency distribution (which has exponent $\gamma = 1 + 1/\rankdistexponent$) and approximating $\genharmonicsum{\Ndistincttypes}{\rankdistexponent}$ by Eq.~\eqref{eq:simple-type-token.genharmonicsum-approx}. 
\item
  Here, we have achieved a direct and compact derivation which proceeds exclusively from the count-rank representation.  
\end{textblock}

  
\begin{textblock}
\item 
  However, Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu}
  is incorrect for large $\rankdistexponent$,
  and the error is in the 
  integral approximation of
  Eq.~\eqref{eq:simple-type-token.genharmonicsum-approx} (which we explain below).
\item 
    We return to Eq.~\eqref{eq:simple-type-token.type-token-relationship},
    and instead use the Euler-Maclaurin expansion~\cite{apostol1999} of $\genharmonicsum{\Ndistincttypes}{\rankdistexponent}$ for $\rankdistexponent \neq 1$, i.e.,
    \item 
    \begin{align}
        \genharmonicsum{\Ndistincttypes}{\rankdistexponent} 
        &
        =
        \frac{
        \Ndistincttypes^{1-\rankdistexponent}
        }{
        1-\rankdistexponent
        }
        +
        \zeta(\rankdistexponent)
        +
        \frac{1}{2} \Ndistincttypes^{-\rankdistexponent}
        \\
        \notag
        &-
        \frac{
        \rankdistexponent
        }{
        12 
        }
        \Ndistincttypes^{-\rankdistexponent-1}
        +
        \mathcal{O}\left(
        \Ndistincttypes^{-\rankdistexponent-2}\right).
    \end{align}
    
    \item
We now have
\item
    \begin{equation}
        \rgrtime \simeq 
        \frac{
        \Ndistincttypes
        }{
        1-\rankdistexponent
        }
        +
        \Ndistincttypes^\rankdistexponent \zeta(\rankdistexponent)
        +
        \frac{1}{2}
        -
        \frac{
        \rankdistexponent
        }{
        12 
        \Ndistincttypes
        } 
        +
        \mathcal{O}
        \left(
        \frac{
        1}{
        \Ndistincttypes^{2}
        }
        \right),
        \label{eq:simple-type-token.type-token-expansion-general-big}
    \end{equation}
    \item
which, to leading order, yields
\item
    \begin{equation}
        t
        \sim
        \frac{
        1
        }{
        1-\rankdistexponent
        }
        \Ndistincttypes
        +
        \zeta(\rankdistexponent)
        \Ndistincttypes^{\rankdistexponent},
        \label{eq:simple-type-token.type-token-expansion-general}
    \end{equation}
    \item
    where
    $\zeta(\rankdistexponent)$ is the Riemann zeta function for $\rankdistexponent > 1$ and its analytical continuation for $\rankdistexponent < 1$. 
\end{textblock}

\begin{textblock}
    In panels Fig.~\ref{fig:simple-type-token.type_token_fit} a)--f), we show how Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} fits the behavior of Eq.~\eqref{eq:simple-type-token.type-token-relationship} for five example values of $\rankdistexponent$. 
    \item
    As we show in the following, we can invert the limiting form of Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} for certain values and ranges of $\rankdistexponent$ and compute $\Ndistincttypes(\rgrtime)$
    as a function of
    $\rgrtime$.
\end{textblock}

\begin{figure*}[t]
\centering
  \includegraphics[width=0.9\textwidth]{figures/localized/samples_yeseq.png}
    \caption{Comparison between data discretely generated using the harmonic sum in Eq.~\eqref{eq:simple-type-token.type-token-relationship} and the results yielded both by the expansion in Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} and by Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu} for different values of $\rankdistexponent$. In c), Eq.~\eqref{eq:simple-type-token.token-type-scaling-behavior} for $\alpha = 1$ is used to solve the divergence. In e) and f), we show the deviation of Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu} from the data in the $\rankdistexponent \gg 1$ regime. 
    }
  \label{fig:simple-type-token.type_token_fit}
\end{figure*}

% \section*{Limiting behavior}

\begin{textblock}
\item
  \textit{Limiting behavior}---For large 
  $\rgrtime$ 
  and 
  $\Ndistincttypes$,
  we can express Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} in simpler forms for
  the three regimes of 
  $\rankdistexponent \ll 1$,
  $\rankdistexponent \simeq 1$,
  and
  $\rankdistexponent \gg 1$.
  
\item
  First,
  for $\rankdistexponent \ll 1$, Eq.~\eqref{eq:simple-type-token.type-token-expansion-general-big} yields 
\item 
    \begin{equation}
    \rgrtime
    \sim
    \frac{1}{1-\rankdistexponent} \Ndistincttypes,
    \label{eq:simple-type-token.t-N-lpha<<1}
    \end{equation}
\item 
because
$\Ndistincttypes^{1} 
\gg 
\Ndistincttypes^{\alpha}
$
and
$
\lim\limits_{\rankdistexponent \rightarrow 0} \zeta(\rankdistexponent) 
 = 
 -1/2.
 $
\end{textblock}
 
\begin{textblock}
\item
Second, for $\rankdistexponent \rightarrow 1$, 
we use the approximations
\item
    \begin{equation}
        \Ndistincttypes^{\rankdistexponent} 
        \rightarrow 
        \Ndistincttypes 
        \left[
        1 
        - 
        (1 - \rankdistexponent) 
        \ln \Ndistincttypes 
        +
        \mathcal{O}
        \left(
        (1 - \rankdistexponent)^{2}
        \right)
        \right]
        \label{eq:simple-type-token.Nalpha-leading-order}
    \end{equation}
    \item
    and
    \item
    \begin{equation}
    (1 - \rankdistexponent)
    \zeta(\rankdistexponent) 
    \rightarrow 
    -1
     +
     \gamma_0
     (1 - \rankdistexponent)
     +
     \mathcal{O}
     \left(
     (
     1 - \rankdistexponent
     )^{2}
     \right)
     \label{eq:simple-type-token.zeta-leading-order}
    \end{equation}
    \item
    where
    $\gamma_{0} \simeq 0.577$ 
    is the Euler-Mascheroni constant. 
    \item
    Substituting
    Eqs.~\eqref{eq:simple-type-token.Nalpha-leading-order}
    and~\eqref{eq:simple-type-token.zeta-leading-order}
    into 
    Eq.~\eqref{eq:simple-type-token.type-token-expansion-general}, 
    we have
    for
    $\rankdistexponent
    \rightarrow 
    1$
    that
    \item
    \begin{equation}
        \rgrtime 
        \sim 
        \Ndistincttypes 
        \left(
        \ln 
        \Ndistincttypes 
        +
        \gamma_{0} 
        \right).
        \label{eq:simple-type-token.t-N-alpha=1}
    \end{equation} 
\item
    By next using the leading term of the asymptotic form of the Lambert $\LambertW$ function, we obtain
    \begin{equation}
        \Ndistincttypes 
        \sim 
        \frac{
        t
        }{
        \ln 
        \rgrtime
        + 
        \gamma_{0}
        - 
        \ln
    \left(
     \ln 
        \rgrtime
        + 
        \gamma_{0}
    \right)
        }.
    \end{equation}
\item 
Finally, for $\rankdistexponent \gg 1$, the exponential term in Eq.~\eqref{eq:simple-type-token.type-token-expansion-general}
dominates and because 
$\zeta(\rankdistexponent) \rightarrow 1$,
the limiting behavior is given by
\begin{equation}
\rgrtime
\sim
\Ndistincttypes^{\rankdistexponent}.
\end{equation}

\item
We observe that in the regime in which $\rankdistexponent \gg 1$, Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu} 
incorrectly gives $t \rightarrow (\rankdistexponent-1)^{-1} \Ndistincttypes^{\rankdistexponent}$, 
which is off from the actual behavior of Eq.~\eqref{eq:simple-type-token.type-token-relationship} 
by a factor $(\rankdistexponent-1)^{-1}$.
\item
The reason for the error
is that the first term of 
$\genharmonicsum{\Ndistincttypes}{\rankdistexponent}$
is 1,
independent of $\rankdistexponent$,
but the steep decay for high $\rankdistexponent$
means that the integral approximation
of Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu}
estimates it as 
$1/(\rankdistexponent-1)$.
\item
We indicate the error in panels e) and f) of Fig.~\ref{fig:simple-type-token.type_token_fit}
for $\rankdistexponent = 10$ and $\rankdistexponent = 15$, respectively.
\item 
Note that we maintain $(\rankdistexponent-1)^{-1}$ instead 
of $\rankdistexponent^{-1}$ to match our 
simulations for these values of 
$\rankdistexponent$.
\end{textblock}

\begin{textblock}
\item
The above derived limiting forms of Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} 
for 
large
  $\rgrtime$ 
  and 
  $\Ndistincttypes$,
can be summarized as
  \begin{equation}
    \rgrtime
    \sim
    \left\{
    \begin{array}{cl}
      \frac{1}{1-\rankdistexponent} \Ndistincttypes
      &
      \textnormal{for}
      \
      \rankdistexponent \ll 1,
      \\ 
      \Ndistincttypes 
      \left(
      \ln
      \Ndistincttypes 
      + 
      \gamma_{0} 
      \right)
      &
      \textnormal{for}
      \
      \rankdistexponent = 1,
      \\
      \Ndistincttypes^{\rankdistexponent}
      &
      \textnormal{for}
      \
      \rankdistexponent \gg 1,
      \\
    \end{array}
    \right.
    \label{eq:simple-type-token.token-type-scaling-behavior}
  \end{equation}
\item 
    and
  
\item
  \begin{equation}
    \Ndistincttypes
    \rightarrow
    \left\{
    \begin{array}{cl}
      % \rgrtime
      % &
      % \textnormal{for}
      % \
      % \rankdistexponent
      % =
      % 0,
      % \\
      (1-\rankdistexponent) \rgrtime
      &
      \textnormal{for}
      \
      \rankdistexponent \ll 1,
      \\
      \rgrtime/\left[
      \ln 
      \rgrtime
      + 
      \gamma_{0}
      -
      \ln
      \left(
     \ln 
        \rgrtime
        + 
        \gamma_{0}
    \right)
      \right]
      &
      \textnormal{for}
      \
      \rankdistexponent = 1,
      \\
      \rgrtime^{1/\rankdistexponent}
      &
      \textnormal{for}
      \
      \rankdistexponent \gg 1.
    \end{array}
    \right.
    \label{eq:simple-type-token.type-token-scaling-behavior}    
  \end{equation}
\end{textblock}

% \begin{figure*}[t]
% \centering

%   \includegraphics[width=0.8\textwidth]{figures/localized/R2_vs_alpha.png}
  
%   \caption{Goodness of the limits in Eqs.~\eqref{eq:simple-type-token.token-type-scaling-behavior} and \eqref{eq:simple-type-token.type-token-scaling-behavior} evaluated in log-space as a function of the rank exponent $\rankdistexponent$. The data used for the fit corresponds to $10^3$ points ($t$, $N$) for $N \in [10^3, 10^4]$, computed using the sum in Eq.~\eqref{eq:simple-type-token.type-token-relationship}.}


%   \label{fig:simple-type-token.type_token_fit}
  
% \end{figure*}

\begin{textblock}
\item
  While Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} fits the behavior correctly 
  for $\rankdistexponent\neq 1$, 
  the applicability of the simpler expressions for the limits in Eqs.~\eqref{eq:simple-type-token.token-type-scaling-behavior}~and~\eqref{eq:simple-type-token.type-token-scaling-behavior} depends on the range of $\rankdistexponent$, 
  as we demonstrate in Fig.~\ref{fig:simple-type-token.type_token_fit_r2}.
\end{textblock}

\begin{figure}[t]
\centering
  \includegraphics[width=\linewidth]{figures/localized/fits_yeseq.png}
    \caption{Goodness of the fit of the expansion in Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} and the approximations in Eq.~\eqref{eq:simple-type-token.token-type-scaling-behavior}. The data used for the fit corresponds to $10^3$ points for $\Ndistincttypes \in [1, 10^3]$, computed using the sum in Eq.~\eqref{eq:simple-type-token.type-token-relationship}.
    }
  \label{fig:simple-type-token.type_token_fit_r2}
\end{figure}



% \section*{Discussion}

\begin{textblock}
\item 
\textit{Discussion}---In this work, we have presented a simple derivation of the asymptotic behavior of the type–token relationship for growing systems with inverse power-law count rankings.
\item
Our expression for the number of tokens $\rgrtime$ (equivalently system size)
as a function of the number of distinct types
$\Ndistincttypes$
in
Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} 
fully captures large system behavior for all 
$\rankdistexponent \ge 0$.
\item 
Our results extend and correct those of 
\item
L\"{u} \etal~\cite{lu2010a}, 
\item 
achieving a more accurate approximation 
while only requiring count-ranking.
\item
Importantly, because our results follow from an idealized growing model,
Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} is independent of the underlying mechanism that drives real system growth. 
\end{textblock}

\begin{textblock}
\item 
As can be visually appreciated in Fig.~\ref{fig:simple-type-token.type_token_fit}~a)--f), a linear approximation of the type–token relation in log–log space provides an accurate graphical description for any value of $\rankdistexponent$, provided that the system size $t$ is sufficiently large. 
\item
This observation, as discussed in Ref.~\cite{lu2010a}, 
clarifies why Heaps’ law so frequently appears in empirical studies.
\end{textblock}

\begin{textblock}
\item 
Our results demonstrate that Heaps' law is not an independent phenomenon, or one dependent on stochastic growth, but is rather an emergent statistical relationship of growing systems with 
inverse power-law count-rankings.
\end{textblock}




==> simple-derivation-of-the-finite-type-token-law.changelog.tex <==
%% for arXivs of the various stripes

\todo{Notes on what has changed}


==> simple-derivation-of-the-finite-type-token-law.contributions.tex <==
Who did what.


==> simple-derivation-of-the-finite-type-token-law.keywords.tex <==
type-token scaling,
scaling,
size-rank distributions,
Zipf's law,
Heaps' law,
power-law tails,
finite size,
language,
complex systems


==> simple-derivation-of-the-finite-type-token-law.methods.tex <==
\section{Methods}
\label{sec:papertag.methods}






==> simple-derivation-of-the-finite-type-token-law.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}



==> simple-derivation-of-the-finite-type-token-law.outtakes.tex <==
  \item
    Indeed, for certain ranges and values of $\rankdistexponent$, when  $\rgrtime$ and $\Ndistincttypes$ are sufficiently large, Eq.~\eqref{eq:simple-type-token.type-token-relationship} returns a simple type-token scaling law, i.e., Heaps' law~\cite{Chacoma2020}.

\todo{Fix this}
Importantly, we show that 
Eq.~\eqref{eq:simple-type-token.lu-exponents} holds only in the extreme limits of $\rankdistexponent \ll 1$ and $\rankdistexponent \gg 1$, whereas the actual scaling behavior of the number of types with the number of tokens deviates from this form and is described here in a simple and explicit manner.
\item 

In the pathological case of $\rankdistexponent = 1$, we can define $\rankdistexponent = 1+\varepsilon$, with $\varepsilon \ll 1$, and
    \begin{equation}
        \frac{\Ndistincttypes}{1-\rankdistexponent} = -\frac{\Ndistincttypes}{\varepsilon},
    \end{equation}
    \begin{equation}
        \Ndistincttypes^\rankdistexponent  \rightarrow \Ndistincttypes \left[ 1 + \varepsilon \ln \Ndistincttypes +\mathcal{O}\left(\varepsilon^2\right)\right],
    \end{equation}
    \begin{equation}
        \zeta(\rankdistexponent) \rightarrow \frac{1}{\varepsilon}+\gamma+\mathcal{O}\left(\varepsilon\right),
    \end{equation}
    $\gamma\simeq 0.577$ being the Euler-Mascheroni constant. Thus, 
    \begin{equation}
        \rgrtime \sim \Ndistincttypes \left( \ln \Ndistincttypes + \gamma\right).
    \end{equation} 
    
    Using the leading logarithmic term of the asymptotic form of the Lambert $\LambertW$ function, we have that
    \begin{equation}
        \Ndistincttypes \sim \frac{t}{\ln t + \gamma}.
    \end{equation}

\tolerance=1
\emergencystretch=\maxdimen
\hyphenpenalty=10000
\hbadness=10000

\justifying

\section*{Introduction}
\label{sec:simple-type-token.introduction}

Universal statistical regularities play a central role in the study of complex systems. 
Prominent examples are power-law behaviors, such as Zipf’s law for word frequencies~\cite{zipf1946},  observed across human~\cite{altmann2016} and animal~\cite{arnon2025} communication. 
Zipf’s law states that the count of a word in a text decreases with its rank $r$ as $S_{\rank,\rankdistexponent} \sim r^{-\rankdistexponent}$, with $\rankdistexponent \simeq 1$. 
Heavy-tailed patterns of this kind also appear in ecological systems~\cite{yule1925, camacho2001},  in the degree distributions of networks~\cite{Redner1998, barabasi1999},  and in socioeconomic contexts~\cite{serrano2003, pinto2012, gabaix2016, gaillard2023}. 
Another well-known scaling regularity is Heaps’ or Herdan's law for sublinear growth~\cite{herdan1960, heaps1978},  which describes how the vocabulary size $N$ of a text grows with its total length $t$ as $N_{t, \beta} \sim t^{\beta}$,  with $0 < \beta < 1$. 
Heaps-type scaling has also been reported in other domains alongside Zipf’s law,  including chemoinformatics~\cite{benz2008},  computer code~\cite{zhang2009},  and urban systems~\cite{simini2019}.


The fact that Zipf’s and Heaps’ laws are empirically observed to hold simultaneously has motivated interest in whether a fundamental relationship between them exists in finite, real systems. Previous works have developed several different frameworks to relate both scaling laws, for example, by empirical observation~\cite{baeza-yates2000}, proposing specific language models~\cite{zanette2005,serrano2009}, growth dynamics~\cite{laurent2016} or sampling mechanisms~\cite{vanleijenhorst2005, eliazar2011}, or assuming in advance their simultaneous validity~\cite{bernhardsson2009}.

All aforementioned findings relate Zipf's and Heaps' laws for $\alpha > 1$. Interestingly, L\"u \textit{et al.} find in Ref.~\cite{lu2010a} a relation between both scaling exponents given by
\begin{equation}
    \beta = 
    \begin{cases}
        1/\alpha, & \textnormal{for} \ \alpha > 1,\\
        1, & \textnormal{for} \ \alpha < 1.
    \end{cases}
    \label{eq:simple-type-token.lu-exponents}
\end{equation}

\begin{textblock}
\item
Here, we present a simple and general type–token relationship for growing finite systems, valid for any value of the scaling exponent $0\leq \alpha<\infty$.  
\item
The formulation is consistent with previous results, reduces to Heaps' law in specific limits and refines earlier approximations. Importantly, we show that Eq.~\eqref{eq:simple-type-token.lu-exponents} holds only in the extreme limits of $\rankdistexponent \ll 1$ and $\rankdistexponent \gg 1$, whereas the actual scaling behavior of the number of types with the number of tokens deviates from this form and is described here in a simple and explicit manner.
\item 
Our approach is independent of the underlying mechanisms of the system, provides an excellent fit to data from scale-free finite-size systems and offers further insight into the growth dynamics of such systems.
\end{textblock}

\begin{figure*}[t]
\centering

  \includegraphics[width=0.9\textwidth]{figures/localized/samples_and_R2_vs_alpha_combined.png}
  
  \caption{a)--e) Comparison between data discretely generated using the harmonic sum in Eq.~\eqref{eq:simple-type-token.type-token-relationship} and the results yielded both by the expansion in Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} and by Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu} for different values of $\rankdistexponent$. In c), Eq.~\eqref{eq:simple-type-token.token-type-scaling-behavior} for $\alpha = 1$ is used to solve the divergence. In e), we show the deviation of Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu} from the data in the $\rankdistexponent \gg 1$ regime. f) Goodness of the fit of the expansion in Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} and the approximations in Eq.~\eqref{eq:simple-type-token.token-type-scaling-behavior}. The data used for the fit corresponds to $10^3$ points for $\Ndistincttypes \in [1, 10^3]$, computed using the sum in Eq.~\eqref{eq:simple-type-token.type-token-relationship}.}


  \label{fig:simple-type-token.type_token_fit}
  
\end{figure*}

\section*{Type-token law}
\label{sec:simple-type-token.type-token-law}

\begin{textblock}
\item
  We start with an idealized growing system comprising
  countable tokens as instances of types. 
\item
  We set aside physical mechanisms
  and consider a system emerging
  in time as follows.
\item
  The system grows in discrete time  
  so that there are $\rgrtime$ total
  tokens at time $\rgrtime = 1, 2, \ldots$,
  and such that the count of
  the $\rank$th type is
\item
  \begin{equation}
    \typesize_{\rank,\rgrtime,\rankdistexponent}
    =
    \left\lfloor
    \frac{1}{2}
    +
    \growthfactor
    \rank^{-\rankdistexponent}
    \right\rfloor.
    \label{eq:simple-type-token.Srt-base-equation-set-up}
  \end{equation}
\item
  where $\lfloor \cdot \rfloor$
  is the floor operator, converted to a round-to-the-nearest-integer
  operator by the addition of 1/2, 
  and $\growthfactor$ is a growth facter
  which we define below.
\item
  We indicate count by $\typesize$ which stands
  for the more general conception of size.
\item
  By construction, types remain ordered in size ranking
  according to their arrival time.
\item
  When their size first
  rounds up to 1,
  we may consider types as being created or uncovered.
\item
  At any time $t$, there will be a finite number
  $\Ndistincttypesfn{\rgrtime}{\rankdistexponent}$
  of
  types with one or more tokens in the system, $\Ndistincttypesfn{\rgrtime}{\rankdistexponent}$
  being also the rank of
  the most recently arrived type.
\item 
  We will see growing groups of types with token counts tied at
  small group sizes of 1, 2, 3, \ldots
\end{textblock}

\begin{textblock}
\item
  Because the system is a realized entity,
  we call 
  $\typesize_{\rank,\rgrtime,\rankdistexponent}$
  a size-ranking rather than a size-rank distribution,
  which mis-implies, for our model, a sampling process.
\item 
  The growth factor
  $\growthfactor \ge 0$
  grows in a step-wise fashion so that
\item 
  \begin{equation}
    \rgrtime
    =
    \sum_{\rank=1}^{\infty}
    \lfloor
     \frac{1}{2}
     +
    \growthfactor
    \rank^{-\rankdistexponent}
    \rfloor.
    \label{eq:simple-type-token.Srt-base-equation-set-up-prefactor}
  \end{equation}
\end{textblock}

\begin{textblock}
\item
  Now, while our idealized system can be easily grown computationally,
  the floor operator prevents ready analysis.
\item
  We approximate the size-ranking of our model as
\item
  \begin{equation}
    \typesize_{\rank,\rgrtime,\rankdistexponent}
    =
    \left\{
    \begin{array}{ll}
      \typesize_{1,\rgrtime,\rankdistexponent}
      \rank^{-\rankdistexponent}
      &
      \textnormal{for}
      \quad
      1
      \le
      \rank
      \le
      \Ndistincttypes,
      \\
      0
      &
      \textnormal{for}
      \quad
      \rank
      >
      \Ndistincttypes.
    \end{array}
    \right.
    \label{eq:simple-type-token.Srt-approx}
  \end{equation}
  
\item
  Sizes are now fractional and we
  we determine $\typesize_{1,\rgrtime,\rankdistexponent}$ below.
\item 
  We note that in some limits, the approximation may not allow
  us to capture the idealized system,
  particularly as $\alpha \rightarrow 0$, because the continuous form smooths over the discrete, step-wise growth that dominates when the size hierarchy flattens, causing the approximate scaling to fail to represent the actual ranked increments.
\item
  Nevertheless, we will be able to satisfactorily
  connect size-rank scaling
  to type-token scaling.
\end{textblock}

\begin{textblock}
\item
  To maintain the connection to our idealized base model, we enforce two conditions.
\item
  First, when a type first appears it has a size of 1.
\item  
  Setting rank $\rank$ to $\Ndistincttypes$
  in Eq.~\eqref{eq:simple-type-token.Srt-approx},
  we have
\item
  \begin{equation}
    \typesize_{\Ndistincttypes,t,\rankdistexponent}
    =
    1
    =
    \typesize_{1,\rgrtime,\rankdistexponent}
    \Ndistincttypes^{-\rankdistexponent},
    \label{eq:simple-type-token.S1-scaling-set-up}
  \end{equation}
\item
  which means
\item 
  \begin{equation}
    \typesize_{1,\rgrtime,\rankdistexponent}
    \sim
    \Ndistincttypes^{\rankdistexponent}.
    \label{eq:simple-type-token.S1-scaling}
  \end{equation}
\item
  Second, we must have the sum of sizes equal to time $\rgrtime$, so
\item 
  \begin{equation}
    \rgrtime
    =
    \sum_{\rank=1}^{N}
    \typesize_{\rank,\rgrtime,\rankdistexponent}
    \sim 
    \Ndistincttypes^\rankdistexponent 
    \genharmonicsum{\Ndistincttypes}{\rankdistexponent}
    \label{eq:simple-type-token.type-token-relationship}
  \end{equation}
\item 
where
\begin{equation}
    \genharmonicsum{n}{a} 
    =
    \sum_{k=1}^{n} 
    k^{-a}
\end{equation}
\item
is the $n$th generalized harmonic number
of order $a$.
\item
  Eq.~\eqref{eq:simple-type-token.type-token-relationship} implicitly gives us what we call
  the type-token relationship, i.e.,
  how the number of distinct types $N$ grows with the size of the sample, $\rgrtime$. 
  
\item 
    We may approximate the harmonic sum in Eq.~\eqref{eq:simple-type-token.type-token-relationship} by its integral form,
    \begin{equation}
    \genharmonicsum{\Ndistincttypes}{\rankdistexponent} 
    \sim 
    \int_{z=1}^{\Ndistincttypes}
    z^{-\rankdistexponent}
    \dee{z},
    \label{eq:simple-type-token.genharmonicsum-approx}
    \end{equation}
    so we would arrive to
    \begin{equation}
        t \sim \frac{
      \Ndistincttypes^{\rankdistexponent}
    }{
      1 - \rankdistexponent
    }
    \left[
      \Ndistincttypes^{1-\rankdistexponent}
      -
      1
      \right].
      \label{eq:simple-type-token.integral_approximation_Lu}
    \end{equation}
    
  Equation~\eqref{eq:simple-type-token.integral_approximation_Lu} coincides with the result obtained by L\"u~\etal in Ref.~\cite{lu2010a}, where the authors derive the connection between the number of distinct types and the total number of tokens by transforming the size-rank distribution into a size-frequency distribution and approximating $\genharmonicsum{\Ndistincttypes}{\rankdistexponent}$ by Eq.~\eqref{eq:simple-type-token.genharmonicsum-approx}. We present a more direct and compact derivation which proceeds exclusively from the size-rank representation.

  
  \item 
  Let us then depart from Eq.~\eqref{eq:simple-type-token.type-token-relationship} without leveraging the approximation of Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu}.
\end{textblock}

\begin{textblock}
\item 
    We use the Euler-Maclaurin expansion~\cite{apostol1999} of $\genharmonicsum{\Ndistincttypes}{\rankdistexponent}$ for $\rankdistexponent \neq 1$, so that
    \begin{align}
        \genharmonicsum{\Ndistincttypes}{\rankdistexponent} 
        &
        =
        \frac{
        \Ndistincttypes^{1-\rankdistexponent}
        }{
        1-\rankdistexponent
        }
        +
        \zeta(\rankdistexponent)
        +
        \frac{1}{2} \Ndistincttypes^{-\rankdistexponent}
        \\
        \notag
        &-
        \frac{
        \rankdistexponent
        }{
        12 
        }
        \Ndistincttypes^{-\rankdistexponent-1}
        +
        \mathcal{O}\left(
        \Ndistincttypes^{-\rankdistexponent-2}\right),
    \end{align}
which leads to
    \begin{equation}
        \rgrtime \simeq 
        \frac{
        \Ndistincttypes
        }{
        1-\rankdistexponent
        }
        +
        \Ndistincttypes^\rankdistexponent \zeta(\rankdistexponent)
        +
        \frac{1}{2}
        -
        \frac{
        \rankdistexponent
        }{
        12 \Ndistincttypes
        } +
        \mathcal{O}\left(\frac{1}{
        \Ndistincttypes^{2}}\right)
        \label{eq:simple-type-token.type-token-expansion-general-big}
    \end{equation}
asymptotically yielding   
    \begin{equation}
        t
        \sim
        \frac{
        1
        }{
        1-\rankdistexponent
        }
        \Ndistincttypes
        +
        \zeta(\rankdistexponent)
        \Ndistincttypes^\rankdistexponent,
        \label{eq:simple-type-token.type-token-expansion-general}
    \end{equation}
    $\zeta(\rankdistexponent)$ being the Riemann zeta function for $\rankdistexponent > 1$ and its analytical continuation for $\rankdistexponent < 1$. In panels a)--e) in Fig.~\ref{fig:simple-type-token.type_token_fit}, we can see how Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} properly fits the behaviour of Eq.~\eqref{eq:simple-type-token.type-token-relationship}. As we show in the following, we can invert the limiting form of Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} for certain values of $\rankdistexponent$ and compute $\Ndistincttypes(\rgrtime)$. Indeed, for certain ranges and values of $\rankdistexponent$, when  $\rgrtime$ and $\Ndistincttypes$ are sufficiently large, Eq.~\eqref{eq:simple-type-token.type-token-relationship} becomes what is most often referred to as Heaps' or Herdan's law~\cite{Chacoma2020}.

\end{textblock}

% \begin{figure*}[t]

%   \includegraphics[width=0.97\textwidth]{figures/localized/Type-Token.png}
  
%   \caption{Different behaviours of Eq.~\eqref{eq:simple-type-token.type-token-relationship}. When $\rankdistexponent \gg 1$, the type-token law behaves as a sublinear power law, namely the Heaps' law.}


%   \label{fig:simple-type-token.type_token}
  
% \end{figure*}


\section*{Limiting behavior}

\begin{textblock}
      
\item
  For big $t$ and $\Ndistincttypes$,
  we can express Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} in simpler forms in certain limits of $\rankdistexponent$.
  
\item
    For $\rankdistexponent \ll 1$, Eq.~\eqref{eq:simple-type-token.type-token-expansion-general-big} yields $t \sim \Ndistincttypes$ because
    \begin{equation}
        \lim_{\rankdistexponent \rightarrow 0} \zeta(\rankdistexponent) = -1/2.
    \end{equation}
\item 
In the pathological case of $\rankdistexponent = 1$, we can define $\rankdistexponent = 1+\varepsilon$, with $\varepsilon \ll 1$, and
    \begin{equation}
        \frac{\Ndistincttypes}{1-\rankdistexponent} = -\frac{\Ndistincttypes}{\varepsilon},
    \end{equation}
    \begin{equation}
        \Ndistincttypes^\rankdistexponent  \rightarrow \Ndistincttypes \left[ 1 + \varepsilon \ln \Ndistincttypes +\mathcal{O}\left(\varepsilon^2\right)\right],
    \end{equation}
    \begin{equation}
        \zeta(\rankdistexponent) \rightarrow \frac{1}{\varepsilon}+\gamma+\mathcal{O}\left(\varepsilon\right),
    \end{equation}
    $\gamma\simeq 0.577$ being the Euler-Mascheroni constant. Thus, 
    \begin{equation}
        \rgrtime \sim \Ndistincttypes \left( \ln \Ndistincttypes + \gamma\right).
    \end{equation} 
    
    Using the leading logarithmic term of the asymptotic form of the Lambert $\LambertW$ function, we have that
    \begin{equation}
        \Ndistincttypes \sim \frac{t}{\ln t + \gamma}.
    \end{equation}
\item 
In the extreme of $\rankdistexponent \gg 1$, the exponential term dominates and $\zeta(\rankdistexponent) \rightarrow 1$,
so $t \rightarrow \Ndistincttypes^\rankdistexponent$. Notice that, in the regime in which $\rankdistexponent \gg 1$, Eq.~\eqref{eq:simple-type-token.integral_approximation_Lu} yields $t \rightarrow \left(\rankdistexponent-1\right)^{-1} \Ndistincttypes^\rankdistexponent$, which is distant from the actual behavior of Eq.~\eqref{eq:simple-type-token.type-token-relationship} by a factor $\left(\rankdistexponent-1\right)^{-1}$, as seen in panel e) of Fig.~\ref{fig:simple-type-token.type_token_fit}.

\item
The above derived limiting forms of Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} can be summarized as
  \begin{equation}
    \rgrtime
    \rightarrow
    \left\{
    \begin{array}{cl}
      % N
      % &
      % \textnormal{for}
      % \
      % \rankdistexponent
      % =
      % 0,
      %\\
      \Ndistincttypes
      &
      \textnormal{for}
      \
      \rankdistexponent \ll 1,
      \\ 
      \Ndistincttypes \left(
      \ln
      \Ndistincttypes + \gamma \right)
      &
      \textnormal{for}
      \
      \rankdistexponent = 1,
      \\
      \Ndistincttypes^{\rankdistexponent}
      &
      \textnormal{for}
      \
      \rankdistexponent \gg 1,
      \\
    \end{array}
    \right.
    \label{eq:simple-type-token.token-type-scaling-behavior}
  \end{equation}
\item 
    and
  
\item
  \begin{equation}
    \Ndistincttypes
    \rightarrow
    \left\{
    \begin{array}{cl}
      % \rgrtime
      % &
      % \textnormal{for}
      % \
      % \rankdistexponent
      % =
      % 0,
      % \\
      \rgrtime
      &
      \textnormal{for}
      \
      \rankdistexponent \ll 1,
      \\
      t/\left(\ln t + \gamma\right)
      &
      \textnormal{for}
      \
      \rankdistexponent = 1,
      \\
      \rgrtime^{1/\rankdistexponent}
      &
      \textnormal{for}
      \
      \rankdistexponent \gg 1.
    \end{array}
    \right.
    \label{eq:simple-type-token.type-token-scaling-behavior}    
  \end{equation}
\end{textblock}

% \begin{figure*}[t]
% \centering

%   \includegraphics[width=0.8\textwidth]{figures/localized/R2_vs_alpha.png}
  
%   \caption{Goodness of the limits in Eqs.~\eqref{eq:simple-type-token.token-type-scaling-behavior} and \eqref{eq:simple-type-token.type-token-scaling-behavior} evaluated in log-space as a function of the rank exponent $\rankdistexponent$. The data used for the fit corresponds to $10^3$ points ($t$, $N$) for $N \in [10^3, 10^4]$, computed using the sum in Eq.~\eqref{eq:simple-type-token.type-token-relationship}.}


%   \label{fig:simple-type-token.type_token_fit}
  
% \end{figure*}

\begin{textblock}
\item
  While Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} fits the behaviour correctly $\forall \rankdistexponent\neq 1$, the applicability of the simpler expressions for the limits in Eqs.~\eqref{eq:simple-type-token.token-type-scaling-behavior}~and~\eqref{eq:simple-type-token.type-token-scaling-behavior} depends on the range of $\rankdistexponent$, as illustrated in panel f) of Fig.~\ref{fig:simple-type-token.type_token_fit}.
\end{textblock}

% \section*{The importance of sampling}

% Up to this point, our analysis has focused on aggregate samples derived from a power-law size-rank distribution. It is crucial to note that Heaps' law, more generally expressed by Eq.~\eqref{eq:simple-type-token.type-token-expansion-general}, does not necessarily hold within a specific sample, since the elements of that sample could, in principle, be rearranged arbitrarily. The validity of Heaps' law depends on the ordering of observations and is satisfied only under random sampling from a power-law size-rank distribution.

% Accordingly, we examine aggregate segments (or chunks) in which $t$ and $N$ are connected through Eq.~\eqref{eq:simple-type-token.type-token-expansion-general}, and in the limiting cases, through Eqs.~\eqref{eq:simple-type-token.token-type-scaling-behavior} and~\eqref{eq:simple-type-token.type-token-scaling-behavior}. However, this correspondence holds only in an aggregate sense. A chunk containing $t$ tokens possesses a vocabulary size $N$, yet the trajectory of $N(t)$ within the chunk does not necessarily adhere to Eq.~\eqref{eq:simple-type-token.type-token-expansion-general}. This disclaimer is important because Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} may be fulfilled in aggregate samples while not within them. An aggregate sample within which the $t$ elements are randomly sampled from the original scale-free size-rank distribution is equivalent to a set of $t$ chunks of sizes 1, 2, 3, ... $t$.

% The reason for this is that Heaps' law is time-sensitive (if time is to be interpreted as addition of elements to th sample), and is only fulfilled in random samplings from a scale-free size-rank distribution. 

% Earlier studies have proposed methods for deriving Heaps' law from Zipf's law under specific sampling conditions~\cite{vanleijenhorst2005, eliazar2011}. In Appendix~\ref{app:simple-type-token.alternative-heaps}, we present an additional derivation of intra-chunk Heaps' scaling based on random sampling within the chunk.


\section*{Discussion}
\begin{textblock}

\item 
In this work, we have presented a simple yet highly precise derivation for the type–token relation of a growing, scale-free, finite system. Our formulation exposes the implicit connection between the statistical structure of the system and its observable type–token dynamics. Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} yields a compact and comprehensive expression for the scaling of the number of types with the number of tokens in a finite system governed by power-law behavior.

\item 
Importantly, Eq.~\eqref{eq:simple-type-token.type-token-expansion-general} is independent of the underlying mechanism that drives system growth. In this sense, our results refine and extend those of L\"u \etal~\cite{lu2010a}, achieving a more accurate approximation while retaining analytical simplicity.

\item 
As can be visually appreciated in Fig.~\ref{fig:simple-type-token.type_token_fit}~a)--e), a linear approximation of the type–token relation in log–log space provides an accurate graphical description for any value of $\rankdistexponent$, provided that the sample size $t$ is sufficiently large. This observation, as discussed in Ref.~\cite{lu2010a}, clarifies why Heaps’ law so frequently appears in empirical studies.

\item 
Crucially, our results provide yet another clear demonstration that Heaps' law is not an independent phenomenon, but rather an emergent statistical feature of growing systems with size-rank power-law tails.

\end{textblock}




\item
  \begin{equation}
    \typesize_{\rank,\rgrtime,\rankdistexponent}
    =
    \left\lfloor
    \frac{1}{2}
    +
    \growthfactor
    \rank^{-\rankdistexponent}
    \right\rfloor.
    \label{eq:simple-type-token.Srt-base-equation-set-up}
  \end{equation}
\item
  where $\lfloor \cdot \rfloor$
  is the floor operator, converted to a round-to-the-nearest-integer
  operator by the addition of 1/2, and we define $g$ below.


\begin{textblock}
\item 
The growth dynamics of finite-size complex systems often exhibit statistical regularities that take the form of power-law distributions. Two well-known examples are Zipf’s and Heaps’ laws, which are known to be related.
\item
To contribute to the understanding of this relationship, we propose a new and more general derivation for the scaling relation between the number of types (species, unique words) and the total number of observed tokens (organisms, words) for finite-size rank–frequency distributions with power-law tails.
\item 
For specific values of the scaling exponent of the rank–frequency distribution, the limiting behavior of the type-token scaling relation reproduces Heaps’ law.
\item
Our approach relies solely on the form of the size–rank distribution and therefore demonstrates that Heaps’ law can arise directly as a consequence of power-law rank–frequency behavior.
\end{textblock}


\todo{Simulate a system whose distribution follows Zipf. Then sample randomly and in a given order. See how Heaps' law behaves. Do it also in chunks, order the chunks, and see how chunk-wise it's fulfilled but not intra-chunk.}

\item
  We determine how the number of distinct types changes
  as we move from the
  $\rgrindex$th
  to the 
  $(\rgrindex+1)$th
  size-rank distribution:
  \begin{equation}
    1
    =
    (\rgrindex+1)
    -
    \rgrindex
    \sim
    \frac{
    \Ndistincttypesfn{\rgrindex+1}{\rankdistexponent}^{\rankdistexponent}
    }{
      1 - \rankdistexponent
    }
    \left[
      \Ndistincttypesfn{\rgrindex+1}{\rankdistexponent}^{1-\rankdistexponent}
      -
      1
    \right]
    -
    \frac{
      \Ndistincttypesfn{\rgrindex}{\rankdistexponent}^{\rankdistexponent}
    }{
      1 - \rankdistexponent
    }
    \left[
      \Ndistincttypesfn{\rgrindex}{\rankdistexponent}^{1-\rankdistexponent}
      -
      1
    \right].
    \label{eq:rich-get-richer-complete.Ni-change}
  \end{equation}


\item 
  \begin{equation}
    \typeinittime
    \typesize_{\rank,\rgrtime}
    \sim    
    \frac{
      (\rankdistexponent - 1)
      \,
      \rgrtime
    }{
      \rank^{\rankdistexponent}
    },
    \label{eq:rich-get-richer-complete.size-rank-distribuion-high-alpha-full}
  \end{equation}
\end{textblock}
\begin{textblock}
\item
  Because when the $\rank$th type first appears
  at $\typeinittime$,
  it is also the
  $\Ndistincttypes$th type
  at $\typeinittime$,
  we can write
\item 
  \begin{equation}
    \typeinittime
    \propto
    \Ndistincttypesfn{\typeinittime}^{\rankdistexponent}
    \label{eq:rich-get-richer-complete.tinit-Nt}
  \end{equation}
\item
  Interpolating to general $\rgrtime$,
  and inverting,
  we retrieve Heaps' law for
  $
  \rankdistexponent
  \gg
  1
  $:
\item 
  \begin{equation}
    \Ndistincttypes
    \propto
    \rgrtime^{
      \frac{
        1
      }{
        \rankdistexponent
      }
    }.
    \label{eq:rich-get-richer-complete.N-t-highalpha}
  \end{equation}
\item
  Requiring also that
  $
  \typesize_{1,\rgrtime}
  \sim
  \Ndistincttypes^{-\rankdistexponent}
  $
  (Eq.~\ref{eq:rich-get-richer-complete.size-rank-norm-check-low-alpha}),
  we have:
\item
  ?? pears at time $\typeinittime$,
  the number of distinct types at that time is
\item 
  $
  \Ndistincttypesfn{\typeinittime}
  =
  \rank.
  $
\item
  We then obtain the innovation rate's behavior
  for
  $
  \rgrtime
  \rightarrow
  \infty
  $
  and
  $\rankdistexponent
  \gg
  1
  $:
  \end{textblock}
\begin{equation}
  \innovationrate
  =
  \frac{
    \dee \Ndistincttypes
  }{
    \dee \rgrtime
  }
  \propto
  \rgrtime^{
    -
    \left(
    1
    -
    \frac{
      1
    }{
      \rankdistexponent
    }
    \right)
  }
  =
  \Ndistincttypes^{-(\rankdistexponent-1)}.
  \label{eq:rich-get-richer-complete.innovation-rate-high-alpha}
\end{equation}

\todo{Get the right normalization and then construction rho t}



  which correctly gives us Heaps' law for
  $\rankdistexponent \ll 1$:
\item 
  \begin{equation}
    \Ndistincttypes
    \sim
    (1 - \rankdistexponent)
    \rgrtime
    =
    \innovationprob
    \rgrtime
    \label{eq:rich-get-richer-complete.heaps-law-low-alpha}
  \end{equation}


\item
  Substituting for $\rank$ in Eq.~\ref{eq:rich-get-richer-complete.growing-initiation-time},
  interpolating to general $\rgrtime$,
  and inverting,
  we retrieve Heaps' law for
  $
  \rankdistexponent
  \gg
  1
  $:
\item 
\begin{equation}
  \Ndistincttypes
  \propto
  \rgrtime^{
    \frac{
      1
    }{
      \rankdistexponent
    }
  }.
  \label{eq:rich-get-richer-complete.N-t-highalpha}
\end{equation}


\item 
\begin{equation}
  \typeinittime
  \sim
  \frac{
    \rgrtime
  }{
    \Ndistincttypesfn{\typeinittime}
  }
  \rank^{\rankdistexponent}
  \
  \textnormal{for}
  \
  \rankdistexponent
  \gg
  1.
  \label{eq:rich-get-richer-complete.growing-initiation-time}
\end{equation}


\begin{textblock}
\item
  We write the number of distinct types at time
  $\rgrtime$
  as
  $\Ndistincttypes$.
\item
  
\item
\end{textblock}
\begin{equation}
  \Ndistincttypes
  \propto
  \rgrtime^{\Ntypesexponent}
  =
  \left\{
  \begin{array}{l}
    \rgrtime^{1}
    \,
    \textnormal{for}
    \,
    \rankdistexponent \le 1,
    \\
    \rgrtime^{1/\rankdistexponent}
    \,
    \textnormal{for}
    \,
    \rankdistexponent > 1.
  \end{array}
  \right.
  \label{eq:rich-get-richer-complete.heaps-law}
\end{equation}

